Humans as a Calibration Pattern: Dynamic 3D Scene Reconstruction from Unsynchronized and Uncalibrated Videos

Recent works on dynamic 3D neural field reconstruction assume the input from synchronized multi-view videos whose poses are known. The input constraints are often not satisfied in real-world setups, making the approach impractical. We show that unsynchronized videos from unknown poses can generate dynamic neural fields as long as the videos capture human motion. Humans are one of the most common dynamic subjects captured in videos, and their shapes and poses can be estimated using state-of-the-art libraries. While noisy, the estimated human shape and pose parameters provide a decent initialization point to start the highly non-convex and under-constrained problem of training a consistent dynamic neural representation. Given the shape and pose parameters of humans in individual frames, we formulate methods to calculate the time offsets between videos, followed by camera pose estimations that analyze the 3D joint positions. Then, we train the dynamic neural fields employing multiresolution grids while we concurrently refine both time offsets and camera poses. The setup still involves optimizing many parameters; therefore, we introduce a robust progressive learning strategy to stabilize the process. Experiments show that our approach achieves accurate spatio-temporal calibration and high-quality scene reconstruction in challenging conditions.

==> algorithms/align_time.tex <==

\DontPrintSemicolon
% \newcommand\algcommentfont[1]{\footnotesize\textcolor{MidnightBlue!80!Gray}{#1}}
\SetCommentSty{algcommentfont}
\SetKwFunction{KwFn}{Fn}
\SetKw{Continue}{continue}
\SetNlSty{}{}{}

\begin{algorithm}[t]
    % \small
    \footnotesize
    % \setstretch{0.95}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwProg{Func}{Function}{:}{end}
    \Func{\sc Global Align($\mathbf{H})$}{
        \SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \Input{Unsynchronized human motions $\mathbf{H}=\{\mathbf{H}^i\}$}
        \Output{Globally aligning time offsets $\Delta t\in\mathbb{Z}^N$}
        % \BlankLine
        Globally aligning time offsets $\Delta t=\mathbf{0}\in\mathbb{Z}^N$\;
        Globally aligned index group $\mathbf{G} = \varnothing$\;
        Locally aligned index group list $\mathbf{G}_{l}=\varnothing$\;
        ${C}, \Delta{T} \gets \text{\sc All-Pair DTW}(\mathbf{H}) $ \;
        index list $\mathbf{I} = \{(i,j)\vert \forall i<j\}$\;
        $\mathbf{I}\gets \text{\sc Sort}(\mathbf{I})$\Comment{increasing order w.r.t. ${C}_{ij}$}\;
        $(i,j)\gets \mathbf{I}[0]$\Comment{anchor indices}\;
        $\Delta t[i] \gets 0, \Delta t[j] \gets \Delta{T}_{ij}$\;
        Insert $(i,j)$ to $\mathbf{G}$\;
        \For{$k=\{1,\cdots,N(N-1)/2-1\}$}{
            $(i,j)\gets \mathbf{I}[k]$\;
            \uIf{$i\in\mathbf{G}, j\in\mathbf{G}$}{
                \Continue
            }
            \uElseIf{$i\in\mathbf{G}, j\in\mathbf{G}_{{l}}[k],\exists k$}{
                Pop $\mathbf{G}_{{l}}[k]$ and add to $\mathbf{G}$ after shift $\Delta{T}_{ij}$\;
            }
            \uElseIf{$i\in\mathbf{G},j\notin\mathbf{G},j\notin\mathbf{G}_{{l}}[k],\forall k$}{
                Add $j$ to $\mathbf{G}, \Delta{t}[j]\gets \Delta{t}[i] + \Delta{T}_{ij}$\;
            }
            \uElseIf{$i\in\mathbf{G}_{l}[k], j\notin\mathbf{G},j\notin\mathbf{G}[l],\forall l$}{
                Add $j$ to $\mathbf{G}_{{l}}[k]$, $\Delta{t}[j]\gets \Delta t[i] + \Delta{T}_{ij}$\;
            }
            \uElseIf{$i,j\notin\mathbf{G},\notin\mathbf{G}_{l}[k],\forall k$}{
                Add $(i,j)$ to new group in $\mathbf{G}_{{l}}$\;
                $\Delta{t}[i]\gets 0, \Delta{t}[j]\gets \Delta\mathbf{T}_{ij}$\;
            }
            \uElseIf{$i\in\mathbf{G}_{l}[k],j\in\mathbf{G}_{l}[l]$}{
                Pop $\mathbf{G}_{l}[l]$ and add to $\mathbf{G}_{l}[k]$ after shift $\Delta{T}_{ij}$\;
            }
            \uElseIf{$i,j\in\mathbf{G}_{l}[k]$}{
                \Continue
            }
            \Else{
                vice versa for reverse case of $(i,j)$\;
            }
        }
        \KwRet $\Delta t$
    }
    \BlankLine
    \Func{\sc All-Pair DTW($\mathbf{H})$}{
        \SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \Input{Human motions $\mathbf{H}$}
        \Output{cost matrix $C\in\mathbb{R}^{N\times N}$, \newline time offset matrix $\Delta{T}\in\mathbb{Z}^{N\times N}$}
        % \BlankLine
        ${C}, \Delta{T}\gets \infty$\;
        \For{$i=\{1,\dots,N\}$}{
            \For{$j=\{i+1,\dots,N\}$}{
                $c, \Delta t = \text{\sc DTW}(\mathbf{H}^i,\mathbf{H}^j,\text{dist type}=\text{\cref{eq:human_dist}})$\;
                ${C}_{ij} \gets c, \Delta{T}_{ij} \gets \Delta t$\;
            }
        }
        \KwRet ${C}$, $\Delta{T}$
    }
    \caption{Time offset estimation \todo{simplify!}}
    \label{alg:align_time}
\end{algorithm}


==> rebuttal_tables/pose_accuracy.tex <==

\begin{table}[b]
    \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{l|c|c|cc}
    \toprule
    \multirow{2}{*}{Experiments} & Rotation ($^\circ$) & Trans.& \multicolumn{2}{c}{$\Delta t$ (frames)}\\
    % \cmidrule{2-7}
    & Init (Refine) & Init (Refine) & Data & Init (Refine)\\
    \midrule
    Mobile-Stage & 5.65 (1.71) & 0.053 (0.002) & 0 & 0.46 (0.21)\\
    EgoBody & 16.8 ($\cdot$) & 0.058 ($\cdot$) & 0 & 1.67 ($\cdot$)\\
    \midrule
    Full dataset & 4.59 ($\cdot$) & 22.7 ($\cdot$) cm & 68.87 & 1.96 ($\cdot$) \\
    \# Cameras$=20$  & 3.74 ($\cdot$) & 18.3 ($\cdot$) cm & 68.87 & 2.24 ($\cdot$)\\
    \# Cameras$=15$  & 3.96 ($\cdot$) & 16.9 ($\cdot$) cm & 68.87 & 0.67 ($\cdot$)\\
    \# Cameras$=10$  & 4.11 ($\cdot$) & 16.1 ($\cdot$) cm & 68.87 & 1.10 ($\cdot$)\\
    \# Cameras$=5$  & 4.31 ($\cdot$) & 12.7 ($\cdot$) cm & 68.87 & 1.12 ($\cdot$)\\
    Mixed framerates & 6.62 ($\cdot$) & 32.7 ($\cdot$) cm & 68.87 & 2.80 ($\cdot$)\\
    \bottomrule
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:rebuttal_align_accuracy}
\end{table}

==> rebuttal_tables/rebuttal_table.tex <==
\begin{table}[t]
\begin{subtable}{0.58\linewidth}
    \centering
    
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l|c|c|c@{}}
    
    \toprule
    \multirow{2}{*}{Experiments} & Rotation ($^\circ$) & Trans.& $\Delta t$ (frames)\\
    % \cmidrule{2-7}
    & Init (Refine) & Init (Refine) &  Init (Refine)\\
    \midrule
    Mobile-Stage & 5.65 (1.71) & 0.053 (0.002) & 0.46 (0.21)\\
    EgoBody & 10.84 ($\cdot$) & 0.034 ($\cdot$) & 1.67 ($\cdot$)\\
    \midrule
    Full dataset & 4.59 ($\cdot$) & 22.7 ($\cdot$) cm & 1.96 ($\cdot$) \\
    \# Cams$=20$  & 3.74 ($\cdot$) & 18.3 ($\cdot$) cm &2.24 ($\cdot$)\\
    \# Cams$=15$  & 3.96 ($\cdot$) & 16.9 ($\cdot$) cm &0.67 ($\cdot$)\\
    \# Cams$=10$  & 4.11 ($\cdot$) & 16.1 ($\cdot$) cm &1.10 ($\cdot$)\\
    \# Cams$=5$  & 4.31 ($\cdot$) & 12.7 ($\cdot$) cm & 1.12 ($\cdot$)\\
    Mixed fps & 6.62 ($\cdot$) & 32.7 ($\cdot$) cm & 2.80 ($\cdot$)\\
    \bottomrule
    \end{tabular}
    }
    \caption{Camera parameter estimation results.}
\end{subtable}
\begin{subtable}{0.37\linewidth}
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l|ccc@{}}
    \toprule
    & PSNR & SSIM & LPIPS\\
    \midrule
    Sync-NeRF & 17.26 & 0.410 & 0.284 \\
    Ours & \textbf{23.27} & \textbf{0.816} & \textbf{0.089} \\
    Oracle & 22.98 & 0.806 & 0.093\\
    \bottomrule
    \end{tabular}
   } 
   \caption{\scriptsize View synthesis results.}
\end{subtable}
\vspace{-1em}
\caption{Quantitative results on various experiments. We set the size of bounding box as 1 to measure translation error for Mobile-Stage and EgoBody dataset since we don't know the metric scale.}
\vspace{-1.8em}
\label{tab:rebuttal_table}
\end{table}

==> rebuttal_tables/view_synthesis.tex <==

\begin{table}[b]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{ccc|ccc|ccc}
    \toprule
    \multicolumn{3}{c|}{Sync-NeRF w/ GT pose}  & \multicolumn{3}{c|}{Ours} & \multicolumn{3}{c}{Oracle (GT pose \& time)}\\
    % \cmidrule{2-16}
     PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS\\
    \midrule
    17.26 & 0.410 & 0.284 & \textbf{23.27} & \textbf{0.816} & \textbf{0.089} & 22.98 & 0.806 & 0.093\\
    \bottomrule
    \end{tabular}
    }
    % \caption{Quantitative results of novel view synthesis on Mobile-Stage dataset.}
    \caption{Quantitative results on Mobile-Stage dataset.}
    \label{tab:mobile-stage_rendering}
\end{table}

==> tables/smpl_robustness.tex <==

\begin{table}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc}
    \toprule
    \textsc{Tennis} scene & Rotation ($^\circ$) & Trans.(cm) & $\Delta t$ (frames) \\
    \midrule
    L2 norm, $\beta, \Theta$ & 5.382 & 26.130 & 2.100 \\
    Degraded video & 6.496 & 32.374 & 1.133 \\
    SMPL noise, $\sigma=0.01$ & 5.266 & 25.844 & 1.633 \\
    SMPL noise, $\sigma=0.02$ & 5.307 & 25.825 & 0.533 \\
    SMPL noise, $\sigma=0.05$ & 5.310  & 25.861 & 0.833 \\
    SMPL noise, $\sigma=0.1$ & 5.241 & 25.383 & 2.100 \\
    SMPL noise, $\sigma=0.2$ & 5.404 & 26.831 & 2.367 \\
    \midrule
    Default setup & 5.293 & 25.827 & 0.467 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Quantitative results with input degradation, noised human motion estimation, and different choice of human state distance.}
    \label{tab:robustness}
\end{table}
